Sigma Worksheet: Interactive Construction of OLAP Queries

The new generation of cloud data warehouses (CDWs) brings large amounts of data and compute power closer to users in enterprises. The ability to directly access the warehouse data, interactively analyze and explore it at scale can empower users to improve their decision making cycles. However, existing tools for analyzing data in CDWs are either limited in ad-hoc transformations or difficult to use for business users, the largest user segment in enterprises. Here we introduce Sigma Worksheet, a new interactive system that enables users to easily perform ad-hoc visual analysis of data in CDWs at scale. For this, Sigma Worksheet provides an accessible spreadsheet-like interface for data analysis through direct manipulation. Sigma Worksheet dynamically constructs matching SQL queries from user interactions on this familiar interface, building on the versatility and expressivity of SQL. Sigma Worksheet executes constructed queries directly on CDWs, leveraging the superior characteristics of the new generation CDWs, including scalability. To evaluate Sigma Worksheet, we first demonstrate its expressivity through two real life use cases, cohort analysis and sessionization. We then measure the performance of the Worksheet generated queries with a set of experiments using the TPC-H benchmark. Results show the performance of our compiled SQL queries is comparable to that of the reference queries of the benchmark. Finally, to assess the usefulness of Sigma Worksheet in deployment, we elicit feedback through a 100-person survey followed by a semi-structured interview study with 70 participants. We find that Sigma Worksheet is easier to use and learn, improving the productivity of users. Our findings also suggest Sigma Worksheet can further improve user experience by providing guidance to users at various steps of data analysis.

==> generation.tex <==
\section{SQL Query Generation}\label{sec:generation}

The issue of query construction is of great interest to us as an OLAP
system. Although the data warehouses we target are capable of
efficient and speedy query execution, a poorly constructed query can
still fail to benefit from these capabilities. As such, the benefits
of our visual interface may be lost if we are unable to construct
queries whose execution requirements do not meet the resource or
latency constraints of our users. In this section we detail the
considerations that guide our query generation.

\subsection{Key Considerations}

In order to meet our goal of composability, we generate and execute a
single query when producing results for a worksheet. This ensures that
a worksheet remains analogous to a SQL \sql{VIEW}. Furthermore, the
schema of the results we produce may not contain nested relations;
this is partly for practical reasons, as nested relations are not
currently standardized across commercial vendors. This means that any
nesting exposed in the worksheet interface must be virtualized.
However in our experience, these constraints have not worked against
our need to construct optimal queries: issuing multiple queries for a
single worksheet can result in the recomputation of expensive common
subexpressions and \sql{nest} / \sql{unnest} operations can negatively
impact performance, respectively. Finally, optimizing for a particular
database execution engine's behavior may come at the cost of less-than
optimal generation for another, while the task of having separate,
optimized generation for each database is a large engineering
undertaking. Therefore we consider all databases equal in our query
generation. While this assumption does not always hold, we've found
those cases typically arise when the complexity of a generated query
is relatively high: for the user, this presents a tradeoff between
constructing a complex query through direct manipulation or writing,
testing, and highly optimizing that query manually. We've observed
that when given the choice, users tend to prefer the former.

\subsection{FROM and JOIN}

The primary input and joins defined in the worksheet correspond to the
\sql{FROM} and \sql{JOIN} clauses in SQL. When the input is a table or view
reference, the qualified name is used, and inline SQL is rendered as a
subquery. When the input is another worksheet, SQL must be recursively
generated and rendered as a subquery. In some cases common table
expressions (CTEs) are used when the same input is referenced multiple
times in a query.

\subsection{Scalar Expressions}

Expressions that do not contain aggregate or window functions, or
cross-level column references can be trivially translated into SQL. In
some cases, discrepancies between dialects or inconsistent behavior
require special translation. Thus when translating a formula such as
\sling{DateDiff("months",\linebreak[4]\,[start],\,[end])}, the
expression generated for Postgres is different from other databases,
as its dialect does not natively support a \sql{DATEDIFF} function.

\subsection{Aggregates and Windows}

The worksheet's dimension hierarchy is advantageous to query
generation, since it defines a static partitioning and sorting for
each level. This greatly simplifies the translation of aggregate and
window expressions, since it dictates the keys for the \sql{GROUP BY}
clause, as well as the partitioning and sorting for then
\sql{OVER} / \sql{WINDOW} clause.

\subsection{Column References}

Since a formula can reference columns outside of its column's level,
additional steps must be taken to generate an appropriate query. When
a reference refers to a column in an upper level, the functional
dependency between the level keys in the dimension hierarchy can be
used to correlate the appropriate value with rows in the calculation
level. When a references refers to a column in a lower level however,
a similar correlation must produce a single value, given our
constraint that nested relations may not be present in our output
schema. As such, an expression is constructed that determines whether
or not the set of nested values is a singleton set; if this is the
case, that value is made available to downstream calculations; if it's
not, then the resulting value is set to \sling{Null}. In both cases,
an internal annotation is added and passed along to the client, so
that a visual error indicator can be displayed in the case of a
non-singleton set.

\subsection{Filters}

Worksheet filters are fairly simple to translate, as they are
guaranteed to be scalar expressions. The relative order of filters and
expressions in the generated query is always greedy: as soon as a
filter expression's references are available in the query, the filter
is rendered. However the level of the dimensional hierarchy in which
the filtered column resides adds a twist to filter translation, as the
predicate may need to be applied to other levels in the hierarchy.
After a filter is applied in its column's level, we must also apply
it to every other level that contains dependent rows. For example,
imagine a worksheet that contains a base level with columns for
product name and product category, and an upper level (L1) with a key
of product category and a column for product revenue. If a filter is
used to select product categories in (L1) that exceed a specific
revenue threshold, then those product names and categories must also
be selected in the base level.
